Cloud-Edge Training Architecture for Sim-to-Real Deep Reinforcement Learning

Deep reinforcement learning (DRL) is a promising approach to solve complex control tasks by learning policies through interactions with the environment. However, the training of DRL policies requires large amounts of training experiences, making it impractical to learn the policy directly on physical systems. Sim-to-real approaches leverage simulations to pretrain DRL policies and then deploy them in the real world. Unfortunately, the direct real-world deployment of pretrained policies usually suffers from performance deterioration due to the different dynamics, known as the reality gap. Recent sim-to-real methods, such as domain randomization and domain adaptation, focus on improving the robustness of the pretrained agents. Nevertheless, the simulation-trained policies often need to be tuned with real-world data to reach optimal performance, which is challenging due to the high cost of real-world samples. This work proposes a distributed cloud-edge architecture to train DRL agents in the real world in real-time. In the architecture, the inference and training are assigned to the edge and cloud, separating the real-time control loop from the computationally expensive training loop. To overcome the reality gap, our architecture exploits sim-to-real transfer strategies to continue the training of simulation-pretrained agents on a physical system. We demonstrate its applicability on a physical inverted-pendulum control system, analyzing critical parameters. The real-world experiments show that our architecture can adapt the pretrained DRL agents to unseen dynamics consistently and efficiently.

==> sections/related_work.tex <==
\section{Related Work}

\subsection{Sim-to-real}
The current sim-to-real approaches mainly work on training in the simulation and directly deploy the pre-trained agents to the real world, which usually suffer from the reality gap due to the dynamics divergence \cite{neunert2017off}. To mitigate the reality gap, the recent progresses lie in domain randomization \cite{Peng2018} \cite{Sadeghi2016} \cite{andrychowicz2020learning}, domain adaptation  \cite{Finn2017} \cite{rakelly2019efficient} \cite{Yu2020} \cite{James2019} and training with preciser simulations \cite{Tan2018}. 

Domain randomization randomizes the environment settings in the simulation, under which the real-world environment can be regarded as one of the randomized scenarios. After training in the simulation with environmental variations, the pre-trained agent can be directly deployed in the real world. Peng et al. \cite{Peng2018} explored the randomization of dynamic parameters such as Mass, Damping in the simulation for object pushing tasks using a robotic arm. The simulation-learned policy can maintain a similar performance when deployed on a real robot. Sadeghi et al. \cite{Sadeghi2016} trained a DRL policy for quadrotor collision avoidance control with raw monocular images input of randomized rendering settings, and the pre-trained policy can be generalized to the real world without further real-world fine-tuning. The problem with domain randomization is that the learned policy is not the optimal solution but a robust one. Moreover, the performance can not be further improved after being deployed in the real world.

Domain adaptation can be categorized into two main branches: gradient-based meta-learning approach \cite{Finn2017} \cite{rakelly2019efficient} and latent-space based adaptation \cite{Yu2020} \cite{James2019}. Gradient-based meta reinforcement learning policy is to leverage then meta-learner to pre-learn a policy on a large number of different tasks \cite{Finn2017}. When applying the pre-learned meta-policy to the new environment, the policy can adapt to the unseen environment after a few gradient steps tuning with a handful of real-world data. During the adaptation, the policy is usually adapted by learning from the real-world experiences with on-policy algorithms, which is sample inefficient. Rakelly et al. \cite{rakelly2019efficient} combine meta-reinforcement learning with an off-policy algorithm and take probabilistic context variables as part of the input, such that the agent can sense the dynamics changes to speed up the exploration and adaptation in the real world. 
\todo[inline]{Short summary}
\todo[inline]{Check the description of latent representations}
The latent-space-based approaches first learn the policy on latent representations. After being deployed in the unseen environment, the policy can be slightly fine-tuned to adapt to the new dynamics. In \cite{Yu2020}, Yu et al. propose Meta Strategy Optimization (MSO) to training policies with latent variable inputs, which serve as the bias parameters enabling the policy to be generalized to the unseen tasks. When deployed in the real world, the latent variable and the policy networks can be optimized by maximizing the accumulated reward. In the computer vision domain, \cite{James2019} proposes to train a generator converting both the simulated images and real-world images into canonical images, on which the policy can be trained. The real-world experiment shows that the learned policy from the simulation outperforms the domain randomization approaches in a robotic grasping task. The problem with the latent-space-based adaptation approaches is that the latent inference model may produce non-optimal results due to the notable dynamics change.

Training with preciser simulations is a direct way to narrow the reality gap where the agents can be trained with more accurate physical properties. In \cite{Tan2018} the system identification is performed to find the correct dynamic parameters, and the actuator and latency are also well modeled. After training in the accurate simulation with domain randomization, the learned policy can successfully perform trotting and galloping gaits in the real world. The problem with training in precise simulation is that the system identification and modeling are expensive, which is also not practical for complex systems. 

Besides, Chiang et al. \cite{Chiang2019} propose AutoRL to automate the search for both shaped reward and the neural network structure. The resulting policies proved more robust to the noise and more generalized when applied to the real-world point-to-point and path-follow navigation tasks. The problem is that large-scale hyperparameters searching is very computationally expensive, even when training in the simulation.


\subsection{Real World Training}
Training DRL agents in the real world from scratch is challenging. The algorithms' inherent instabilities and real-world sampling complexity make the learning of the DRL unstable and even never converging. Recent real-world training work explore improving the algorithms \cite{Haarnoja2018} \cite{haarnoja2018soft}, increasing the sampling efficiency \cite{Kalashnikov2018} \cite{Agarwal2020} \cite{nagabandi2018learning} \cite{Yang2020} and easing the exploration \cite{Bojarski2016} \cite{Vecerik2017} \cite{Wu2019} \cite{Johannink2019} to realise direct training on the real world without the help of the simulation.

Training in the real world needs stable DRL algorithms. Recent state-of-the-art algorithms suffer from the sensitivities to the hyperparameter settings, and some of them need considerable effort to tune \cite{henderson2018deep}. Haarnoja et al. \cite{Haarnoja18} extend the Soft actor-critic algorithm \cite{haarnoja2018soft} to learn a locomotion controller on a real-world Minitaur robot from scratch. With the constrained expected entropy and automatic temperature parameter adjustment, a stable gait can be learned in the real world directly in about two hours. 

Sampling efficiency is crucial to real-world training. Model-free DRL off-policy methods can reuse the samples multiple times and are generally about an order of magnitude more data-efficient than on-policy methods \cite{ibarz2021train}. The work \cite{Kalashnikov2018} leverages 580k off-line real-world grasp attempts to train a deep neural network Q-function to perform closed-loop robotic grasping. After online tuning with a handful of real-world on-policy data, the learned policy can be improved to a success rate of 96\% on challenging unseen objects. The work \cite{Agarwal2020} further investigates the effectiveness of off-line training concerning the dataset size, samples diversity, and algorithm choice. One of the problems with off-line training for standard off-policy methods such as DQN and DDPG is the extrapolation error due to the bootstrapping from actions that lie outside of the training data distribution, and it accumulates via the Bellman backup operator \cite{Kumar2019}, which makes the training process unstable. \cite{Kumar2019} propose a bootstrapping error accumulation reduction algorithm, and \cite{Fujimoto2019} propose batch-constrained RL to constrain the action selection. The bootstrapping errors can also be remedied by training with on-policy interaction with the environment\cite{Fujimoto2019}. 

Model-based RL approaches \cite{nagabandi2018learning} \cite{Yang2020} train a model to mimic the real-world dynamics by leveraging a handful of real-world experiences. The learned model then will be used as the interactive environment to train RL agents. Yang et al. \cite{Yang2020} learn a system model that can predict the next state given the current state-action pair by only using 4.5 minutes collected from the real world. Then the learned model is used to train a decent RL policy for quadruped robot control. However, the common problem with the model-based RL is to learn a precise model for training the policies. Sometimes the learned model needs to be continually evaluated and rectified with more real-world training data.

Safe and efficient exploration is another important consideration when training DRL agents in the real world. The real-world exploration difficulties can be significantly eased by leveraging human demonstrator \cite{Bojarski2016}. In sparse reward settings, the demonstration can significantly decrease the attempts to visit the high reward spaces. Vecerik et al.  \cite{Vecerik2017} propose to collect the demonstrations via a robot kinesthetically force-controlled by a human demonstrator. Furthermore, the RL policies are trained with data sampled from the collected demonstrations along with the actual interactions with prioritized replay strategy\cite{schaul2015prioritized}. Sometimes the perfect demonstrations are hard to collect due to the presence of distraction or human's limited attention.  \cite{Wu2019} proposes a confidence scores approach to learn RL policies from the imperfect demonstrations. Comparably, Johannink et al. \cite{Johannink2019} propose to combine a scripted controller with deep RL methods to solve real-world block assembly tasks involving contacts and unstable objects. The script controller can help explore the environment safely, while the DRL agent can learn to deal with the contact dynamics to finish the assembly task. 

There are also distributed learning systems that enable policy learning in the real world asynchronously \cite{gu2017deep} \cite{Kalashnikov2018} \cite{mnih2016asynchronous}. However, most of them need to set up parallel learning mechanisms with massive devices, which is not applicable in most real-world applications.  

In the asynchronous learning system presented in \cite{Haarnoja2018}, a training job periodically appends the entire observed trajectory and reward signals to the replay buffer, from which the training batch is sampled to update the neural networks. After each training, the optimized policy will be sent to update the policy in a data-collection job. Differently, our remote training architecture double buffers the policy agents on the edge device, decoupling the updating of policy agents and real-time interaction with the environment. Thus the policy agents can be updated more frequently, which is vital for real training to converge faster and in a more stable way, as discussed in section V. 
